Deconstructing What Makes a Good Optimizer for Language Models

Training language models becomes increasingly expensive with scale, prompting numerous attempts to improve optimization efficiency. Despite these efforts, the Adam optimizer remains the most widely used, due to a prevailing view that it is the most effective approach. We aim to compare several optimization algorithms, including SGD, Adafactor, Adam, Lion, and Sophia in the context of autoregressive language modeling across a range of model sizes, hyperparameters, and architecture variants. Our findings indicate that, except for SGD, these algorithms all perform comparably both in their optimal performance and also in terms of how they fare across a wide range of hyperparameter choices. Our results suggest to practitioners that the choice of optimizer can be guided by practical considerations like memory constraints and ease of implementation, as no single algorithm emerged as a clear winner in terms of performance or stability to hyperparameter misspecification. Given our findings, we further dissect these approaches, examining two simplified versions of Adam: a) signed momentum (Signum) which we see recovers both the performance and hyperparameter stability of Adam and b) Adalayer, a layerwise variant of Adam which we introduce to study the impact on Adam's preconditioning for different layers of the network. Examining Adalayer leads us to the conclusion that, perhaps surprisingly, adaptivity on both the last layer and LayerNorm parameters in particular are necessary for retaining performance and stability to learning rate.

==> 5_adalayer.tex <==
\section{Investigating the key factors for optimizer stability and performance}
\label{sec:novograd_investigation}

Ablations in the previous section revealed the striking similarity in performance and stability across multiple optimizers compared to Adam. In this section we seek a finer-grained understanding of the role of preconditioning for adaptive optimizers in achieving \emph{both} performance and stability. Adam and its other variants are designed to have a high degree of adaptivity at a fine granularity (per-parameter learning rates) throughout the training process. This adaptivity is often credited with the stability and robust performance observed in these optimizers. However, a critical question arises: to what extent is this adaptivity needed for different parameters of the network? By dissecting the fundamental components that ensure both performance and stability, we aim to discern whether simpler optimizers like SGD can achieve similar benefits with minimal modifications. Since higher momentum can often play the same role as a better preconditioner and to have all algorithms on an equal footing, we will fix $\beta_1 = 0.9$ for all optimizers in this section.

The main optimizer we study in this section is a ``layer-wise'' variant of Adam, which we coin as `Adalayer'.  We use Adalayer for our investigations because it lends a greater ease of understanding compared to full-fledged Adam in identifying parts of the network which may be particularly critical for optimizer performance and stability. Note that this layerwise variant is a special case of a previously known optimizer called Blockwise Adaptive Gradient with Momentum (BAGM) \citep{bagm}.

\subsection{Adalayer}
\label{subsec:lastlayer_correction}


\begin{wrapfigure}[13]{r}{0.55\textwidth}
\begin{minipage}{0.55\textwidth}
\vspace{-1.2cm}
\begin{algorithm}[H]
\SetAlgoNlRelativeSize{-1} %
\SetNlSty{textbf}{\{}{\}} %
\caption{Adalayer \label{alg:adalayer}}
\textbf{Parameters:}
Learning rate $\eta$, exponential decay rates for the moment estimates $\beta_1, \beta_2$, number of steps $T$, $\epsilon$

\While{$t \leq T$}{
    \For{each layer $l$ with $p$ parameters}{
        $g_t^l \gets \nabla_l L(w_t)$ \;
        
        $v_t^l \gets \beta_2 \cdot v_{t-1}^l + (1 - \beta_2) \cdot p^{-1/2} \cdot \|g_t^l\|_2^2$ \;
        
        $m_t^l \gets \beta_1 \cdot m_{t-1}^l + (1-\beta_1)g_t^l$ \;
        
        $w_{t+1}^l \gets w_t^l - \eta \cdot \frac{m_t^l}{\sqrt{v_t^l}+\epsilon}$ \;
    }
}
\end{algorithm}
\end{minipage}
\end{wrapfigure}


To study the behavior of adaptive optimizers like Adam, we begin with describing a layer-wise version of Adam which we refer to as Adalayer. Adam, Adafactor and Adalayer all (approximately) store the diagonal second moment matrix, but with coarser and coarser granularity; for a layer of dimension $m \times n$, Adam explicitly maintains the second moment matrix using $mn$ parameters in the shape of a matrix. Adafactor stores row and column averages of the second moment matrix which serve as a rank-1 approximation to the second moment matrix. Finally, Adalayer stores a single scalar which is the average of the second moment matrix. We will later consider a generalization of Adalayer where instead of averaging second moment over a layer we will average it over a ``block'' of parameters which can be a subset of a layer. We note that similar algorithms have been studied before by ~\citet{ginsburg2019stochastic,grafting} but we choose to study this variant since it is a direct analogue of Adam and Adafactor. A simplified version of Adalayer optimizer is given in Algorithm~\ref{alg:adalayer}, other details such as bias correction are kept same as that for Adam.


\begin{wrapfigure}[14]{r}{0.4\textwidth}
    \vspace{-1cm}
    \captionsetup{belowskip=0pt}
    \includegraphics[width=0.4\textwidth]{images/novograd_freeze/1_novograd.pdf}
    \caption{Modifying Adalayer with the last layer correction improves performance and stability across learning rates.}
    \label{fig:novograd_last_correction}
\end{wrapfigure}


In Figure~\ref{fig:novograd_last_correction} we study the behavior of Adalayer across learning rates. To preserve the correspondence with Adam we fix other hyperparameters to be the same: $\beta_1 = 0.9$, $\beta_2 = 0.95$ and $\epsilon = 1e-15$. We find that Adalayer has better performance than SGD\footnote{Note that in this section we are setting $\beta_1 = 0.9$ for all optimizers.}, but it performs worse than Adam and also lacks Adam's stability across learning rates. The major difference between Adam and Adalayer is the preconditioning done by Adam \textit{within} a layer. Intuitively, this preconditioning will have large effects in layers where we expect different weights within a layer to have different gradient scales. The first candidate for such a layer is the \emph{last layer}, since different tokens have widely different frequencies leading to different gradient scales. To test this hypothesis, we run a corrected version\footnote{We note that this reasoning also applies to the first layer, but in our ablations applying this correction the first layer did not make a significant difference.} of Adalayer where we treat the set of weights feeding into a logit as a separate block. We henceforth refer to Adalayer with this correction as \textbf{Adalayer*}. This is plotted in Figure~\ref{fig:novograd_last_correction} and we observe that Adalayer* almost recovers the performance as well as a large fraction of the stability of Adam. 



To study how Adalayer* preconditions the network, we plot effective learning rates used for different logits by Adalayer* in Figure~\ref{fig:eff-lr-all} (\textbf{Left}). Here, the effective learning rate for a layer $l$ in the network is $\lambda_t / (\sqrt{v^l_t}+\epsilon)$. We find that Adalayer* indeed uses vastly different learning rates for different logits, supporting our hypothesis that preconditioning weight in different logits separately is important for performance and stability.

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{images/effective_learning_rate_quantiles_truncated.pdf}
    \caption{Quantiles of effective learning rates ($\eta_t / (\sqrt{v^l_t}+\epsilon)$ for each layer $l$) for the last layer blocks (\textbf{Left}), the LayerNorm blocks (\textbf{Right}), and the other matrix blocks (\textbf{Middle}) for a 150m model trained using Adalayer*. Unlike the other matrix blocks and LayerNorm parameters, the effective learning rates across logits vary across multiple orders of magnitude, providing evidence for the need to precondition them separately.}
    \label{fig:eff-lr-all}
\end{figure}

